Emergence of radial orientation selectivity: Effect of cell density changes and eccentricity in a layered network

Previous work by Linsker revealed how simple cells can emerge in the absence of structured environmental input, via a self-organisation learning process. He empirically showed the development of spatial-opponent cells driven only by input noise, emerging as a result of structure in the initial synaptic connectivity distribution. To date, a complete set of radial eigenfunctions have not been provided for this multi-layer network. In this paper, the complete set of eigenfunctions and eigenvalues for a three-layered network is for the first time analytically derived. Initially a simplified learning equation is considered for which the homeostatic parameters are set to zero. To extend the eigenfunction analysis to the full learning equation, including non-zero homeostatic parameters, a perturbation analysis is used.

==> eigen_unsymmetricRadius.tex <==

The primary use of a full derivation for the eigenfunctions of Linsker's learning 
equation, is that it may be applied to improve our understanding of learning 
dynamics in a variety of situations. For example, in the event that neural 
density is not isotropic, we can use the same derivation process to understand 
the impact of the anisotropy on learning. To elucidate the value of the derivation, 
we will consider the case in which neural density along the horizontal meridian 
differs to that across the vertical meridian. 

Denote the variance of the Gaussian synaptic density across the horizontal meridian by 
$\radiushoriz{\inputlayer}{\layer{B}}$, and the connection density across the 
vertical meridian by $\radiusvert{\inputlayer}{\layer{B}}$. We can express the 
former as a scaled quantity of the latter, such that 
$\radiushoriz{\inputlayer}{\layer{B}} = \radiusratio \radiusvert{\inputlayer}{\layer{B}}$, 
where $0 < \radiusratio \leq 1$, to indicate a smaller radius across the horizontal 
meridian. In this case the probability of presynaptic neuron, $\preN$, in layer 
\layer{\inputlayer}, generating a synaptic connection to postsynaptic neuron, 
$\postN$, in layer \layer{B}, is given by 
\begin{align}\label{eq:2DUnsymmGauss}
   \probdist{N}{\posx{\preN}{\postN},\posy{\preN}{\postN}}
			   {\vect{0}, \Sigma_{\layer{B}}} 
 &= 
   \frac{1}{\pi\radiushoriz{\inputlayer}{\layer{B}}\radiusvert{\inputlayer}{\layer{B}}} 
   \exp{- \frac{\posx{\preN}{\postN}^2} {\radiushorizvar{\inputlayer}{\layer{B}}}
		+ \frac{\posy{\preN}{\postN}^2} {\radiusvertvar{\inputlayer}{\layer{B}}}} \notag \\
 &= 
   \frac{1}{\pi\radiusratio\radiusvertvar{\inputlayer}{\layer{B}}} 
   \exp{- \frac{\posx{\preN}{\postN}^2} {\radiusratio^2\radiusvertvar{\inputlayer}{\layer{B}}}
		+ \frac{\posy{\preN}{\postN}^2} {\radiusvertvar{\inputlayer}{\layer{B}}}} \notag \\
 &= 
   \frac{1}{\pi\radiusratio\radiusvertvar{\inputlayer}{\layer{B}}} 
   \exp{- \frac{ \posx{\preN}{\postN}^2 
	            +\radiusratio^2 \posy{\preN}{\postN}^2}
	           { \radiusratio^2 \radiusvertvar{\inputlayer}{\layer{B}}} }
\end{align}

Covariance between two layer \layer{B} neurons can easily be shown to be 
\begin{align}
   \scov{\Lrate{\postN}{\layer{B}}{}}{\Lrate{\postNtwo}{\layer{B}}{}}
 &= 
   \frac{ \left( \Rb{\layer{B}}{\layer{C}} \N{\layer{B}}{\layer{C}} \layerstd{\inputlayer} 
		  \right)^2 }
        { 2\pi \radiusratio \radiusvertvar{\inputlayer}{\inputlayer} }
   \exp{-\frac{ \left( \posx{\preN}{\postN} - \posx{\preNtwo}{\postN} \right)^2 
	          + \radiusratio^2 \left( \posy{\preN}{\postN} - \posy{\preNtwo}{\postN} \right)^2 }
			  { 2\radiusvar{\inputlayer}{\layer{B}} } }. 
\end{align}

The continuous learning equation therefore becomes 
\begin{align}\label{eq:learningEqnContAniso}
  \etalayer{} \Lwgtcont{\poscont}{}
 &= \koneAniso{} + 
    \int_{-\infty}^{\infty} \int_{-\infty}^{\infty} 
       \left( \cxcoeffAniso 
			  \exp{- \frac{ \abs{\posxcont -\posxtwocont}^2
			              + \radiusratio^2 \abs{\posycont -\posytwocont}^2} 
				          {2\radiusratio^2\radiusvertvar{\inputlayer}{\layer{A}}}} 
		 	+ \ktwoAniso{} 
	   \right) 
       \exp{- \frac{ \abs{\posxtwocont}^2 
		           + \radiusratio^2 \abs{\posxtwocont}^2 } 
				   { \radiusratio^2 \radiusvertvar{\inputlayer}{\layer{B}}}}
       \Lwgtcont{\colvec{\posxtwocont\\\posytwocont}}{}
	   d\posxtwocont d\posytwocont .
\end{align}

In order to utilise the derivation of eigenfunctions provided, it is necessary to 
introduce a change of variables so that the learning equation describing learning 
with anisotropic connection density has the same format as the learning equation 
given in \eq{\ref{eq:learningEqnCont}}. To this end, introduce a change of variable 
to polar coordinates such that 
$\posrAniso = \posxcont + \radiusratio \posycont$ and 
$\posthAniso = \tan^{-1}\left( \frac{\radiusratio \posycont}{\posxcont} \right) $. 
In this case the learning equation in polar form becomes 

where we have set $\ktwoAniso{}$ to zero for comparability. 
\begin{align}\label{eq:learningEqnContAniso_v2}
  \etalayer{} \Lwgtcont{\poscont}{}
 &= \koneAniso{} + 
    \int_{-\infty}^{\infty} \int_{0}^{2\pi} 
       \left( \cxcoeffAniso 
			  \exp{- \frac{ \posrAniso^2 + \posintrAniso
			              - 2\posrAniso \posintrAniso \cosbr{\posthAniso-\postwothAniso}{} }
				          {2\radiusratio^2\radiusvertvar{\inputlayer}{\layer{A}}}} 
		 	+ \ktwoAniso{} 
	   \right) 
       \exp{- \frac{ \abs{\posxtwocont}^2 
		           + \radiusratio^2 \abs{\posxtwocont}^2 } 
				   { \radiusratio^2\radiusvertvar{\inputlayer}{\layer{B}}}}
       \Lwgtcont{\colvec{\posxtwocont\\\posytwocont}}{}
	   d\posintrAniso d\postwothAniso .
\end{align}



